Rapid radiative clearing of protoplanetary discs

The lack of observed transition discs with inner gas holes of radii greater than ~50AU implies that protoplanetary discs dispersed from the inside out must remove gas from the outer regions rapidly. We investigate the role of photoevaporation in the final clearing of gas from low mass discs with inner holes. In particular, we study the so-called "thermal sweeping" mechanism which results in rapid clearing of the disc. Thermal sweeping was originally thought to arise when the radial and vertical pressure scale lengths at the X-ray heated inner edge of the disc match. We demonstrate that this criterion is not fundamental. Rather, thermal sweeping occurs when the pressure maximum at the inner edge of the dust heated disc falls below the maximum possible pressure of X-ray heated gas (which depends on the local X-ray flux). We derive new critical peak volume and surface density estimates for rapid radiative clearing which, in general, result in rapid dispersal happening less readily than in previous estimates. This less efficient clearing of discs by X-ray driven thermal sweeping leaves open the issue of what mechanism can clear gas from the outer disc sufficiently quickly to explain the non-detection of cold gas around weak line T Tauri stars.

==> diff1 <==
83c83,84
< The lack of observed transition discs with inner gas holes greater than $\sim50$AU in radial extent implies that protoplanetary discs dispersed from the inside out must remove gas from the outer regions rapidly.  We investigate the role of photoevaporation in the final clearing of gas from low mass discs with inner holes. In particular we study the so--called ``thermal sweeping'' mechanism found by Owen et al. (2012): an instability originally thought to arise when the radial and vertical pressure scale heights at the X-ray heated inner edge of the disc match, which results in rapid clearing of the disc. We demonstrate that this criterion is not complete. Rather, rapid clearing depends on the fact that at the disc inner edge a perturbation leading to a reduction in the gas density results in an increase in the gas pressure. This leads to a runaway increase in the X--ray heated pressure up to a maximum possible value and will clear the disc out until the point that this maximum X--ray heated pressure equals the pressure in the cold disc. The criterion for clearing of the whole disc is thus that the peak cold disc pressure is less than that which can be attained in the X--ray heated gas. We derive new critical peak volume and surface density estimates for rapid radiative clearing which, in general, result in rapid dispersal happening less readily than the previous estimate by Owen et al. (2013).  In general, where thermal sweeping initiates is governed by the exponential fall--off in density towards the disc outer edge. For discs with inner holes opened by photoevaporation we find that the maximum possible inner hole radius is about 200\,AU, though clearing happens at considerably smaller radii for stars with mass less than 0.2\,M$_{\odot}$.
---
> The lack of observed transition discs with inner gas holes greater than $\sim50$AU in radial extent implies that protoplanetary discs dispersed from the inside out must remove gas from the outer regions rapidly.  We investigate the role of photoevaporation in the final clearing of gas from low mass discs with inner holes. In particular we study the so--called ``thermal sweeping'' mechanism found by Owen et al. (2012): an instability originally thought to arise when the radial and vertical pressure scale heights at the X-ray heated inner edge of the disc match, which results in rapid clearing of the disc. We demonstrate that this criterion is not fundamental. Rather, rapid clearing initiates when the peak mid--plane volume density would be heated above the local dust temperature if it were optically thin to the X--rays. When this is the case, all optically thin material interior to the peak density will be elevated above the dust temperature. This means that perturbations to the disc inner edge that allow the X--rays to propagate further into the disc will \textit{always} result in further heating, right up to the disc density maximum and beyond. 
> If this is not the case then material becoming optically thin to the X--rays may remain at the dust temperature, suppressing runaway clearing. We derive new critical peak volume and surface density estimates for rapid radiative clearing which, in general, result in rapid dispersal happening much less readily than the previous estimate by Owen et al. (2013).  
109c110,117
< Owen et al. (2012) derived a criterion for thermal sweeping as follows. The radial pressure scale length is $\Delta=dR/d\log{P}$ and the vertical pressure scale length is simply $H=dz/d\log{P}=c_s/\Omega$. In this first model, it is taken that thermal sweeping is initiated when $\Delta=H$. It is assumed that the X-rays penetrate through to the peak surface density of the disc $\Sigma_{\textrm{\textrm{max}}}$. Pressure balance is imposed at the dust and X-ray heated interface
---
> Owen et al. (2012) proposed a criterion for thermal sweeping involving
> equality between the radial pressure scale length in the X-ray heated
> gas   ($\Delta=P/{{d\log{P}}\over{dR}}$ and the local vertical pressure scale length ($H=P/{{d\log{P}\over{dz}}}\sim c_s/\Omega$). In this first model, it is
> assumed that X-rays penetrate through to the surface density peak close to the disc inner
> edge $\Sigma_{\textrm{max}}$. Pressure balance is imposed at the interface
> between the  X-ray heated gas and unperturbed disc gas (in which the temperature
> is set by reprocessing of stellar radiation by dust).  
> 
116c124
< Their analysis then assumes that the radial pressure scale length is actually just the whole column that is optically thin to the X--rays (i.e. $N_{\textrm{X}} = 10^{22}$), in which case 
---
> Their analysis then assumes that the radial pressure scale length is actually just the whole column that is marginally optically thick  to the X--rays (i.e. $N_{\textrm{X}} = 10^{22}$cm$^{-2}$), in which case 
121c129
< We emphasise that this is not strictly the radial pressure scale length ($dR/d\log{P}$).  
---
> We emphasise that this is not strictly the radial pressure scale length ($(d\log P/dR)^{-1}$).   
129c137
< 	\Sigma_{\textrm{\textrm{TS}}} = \sqrt{2\pi} \mu m_H N_{\textrm{X}} \sqrt{\frac{T_{\textrm{X}}}{T_{D}}}
---
> 	\Sigma_{\textrm{TS}} = \sqrt{2\pi} \mu m_H N_{\textrm{X}} \sqrt{\frac{T_{\textrm{X}}}{T_{D}}}
133c141
< 	\Sigma_{\textrm{\textrm{TS}}} = 0.43\textrm{g}\,\textrm{cm}^{-3}\left(\frac{\mu}{2.35}\right)\left(\frac{T_{\textrm{X}}}{400\,K}\right)^{1/2}\left(\frac{T_{D}}{20K}\right)^{-1/2}
---
> 	\Sigma_{\textrm{TS}} = 0.43\textrm{g}\,\textrm{cm}^{-3}\left(\frac{\mu}{2.35}\right)\left(\frac{T_{\textrm{X}}}{400\,K}\right)^{1/2}\left(\frac{T_{D}}{20K}\right)^{-1/2}
143,145c151
< \noindent i) Equation \ref{O122}, i.e. that $n_{\textrm{X}}\Delta$ is always 10$^{22}$ particles (column limited). In reality this column could be lower if the gas is optically thin to the X-rays, but the density is sufficiently high that the X--rays cannot heat the gas above the dust temperature. We refer to this latter scenario as being ``density limited'' \\
< 
< \noindent ii) That the dust to X-ray heated transition occurs at the peak surface density of the disc. It is highly probable that this transition from X--ray heated to dust heated gas will happen at a radial distance from the star interior to the peak surface density radius.  \\
---
> \noindent i) Equation \ref{O122}, that is that $n_{\textrm{X}}\Delta$ is always 10$^{22}$ particles cm$^{-2}$.(column limited). In reality this column could be lower if the gas is optically thin to the X-rays, but the density is sufficiently high that the X-rays cannot heat the gas above the dust temperature. We refer to this latter scenario as being ``density limited'' \\
147c153
< The approach that \cite{2013MNRAS.436.1430O} used was to perform a large number  of 1D simulations (around 5000) with the expected steady state mass loss profile imposed. They then studied how the ratio of $\Delta/H$ varies with the properties of the star-disc system, namely the: stellar mass/X-ray luminosity, peak disc surface density and inner hole radius. They found that the critical peak surface density increases with inner hole radius and X--ray luminosity, which was not accounted for in the initial analytic model. Motivated by these findings they developed an ``improved'' criterion for thermal sweeping that was expected to apply when not in the column limited case. 
---
> \noindent ii) That the dust to X-ray heated transition occurs at the peak surface density of the disc. Instead the  transition from X--ray heated to dust heated gas is located self-consistently at some radius interior to that of  peak surface density. \\
148a155,169
> In recognition of the fact that the flow near the disc rim is nearly
> radial,
>  \cite{2013MNRAS.436.1430O} solved for  1D steady state flows with
> mass loss rates set by conditions at the X-ray sonic surface. Such flows
> are highly subsonic in the vicinity of the disc rim and thus the
> structure in this region (which is important for assessing the onset
> of thermal sweeping in 2D) is close to one of hydrostatic equilibrium. This
> allowed \cite{2013MNRAS.436.1430O} to propose analytic criteria
> for the onset of thermal sweeping (i.e. assuming that this
> occurs when $\Delta = H$) in both
> the density limited and column limited regimes.
>  They found that (in contrast to the hypothesis in Owen et al 2012)
> the X-ray heated interface is generally set by the density limited criterion
> and that in this case the critical peak surface density {\it increases} with inner hole radius and X-ray luminosity. Motivated by these findings they developed an ``improved'' criterion for thermal sweeping which we give below (correcting
> typos in Owen et al (2013):
150,167d170
< This new criterion still assumes that thermal sweeping arises at $\Delta=H$ and is still evaluated by considering pressure balance at the interface of the X-ray and dust heated zones. It differs in that this interface can be arbitrarily located. They found that the new critical surface density for thermal sweeping is
< \begin{equation}
< 	\Sigma_{\textrm{\textrm{TS}}} = \sqrt{2\pi}\frac{P_{\textrm{X}}}{c_c \Omega} \exp\left({\frac{T_{\textrm{X}}}{2T_c}}\right).
< \end{equation}
< where $c_c$ is the sound speed at the centrifugal radius. 
< The heating function used in both  \cite{2012MNRAS.422.1880O} and \cite{2013MNRAS.436.1430O} is  a function of the local ionisation parameter $\xi = L_{\textrm{X}}/(n_{\textrm{X}} D^2)$ (also used here and discussed in more detail in section \ref{ionparam}). At the X-ray interface (the base of the X-ray wind) the ionisation parameter is at its minimum value, which the authors approximated by assuming it is close to that at the pressure maximum that occurs at radius $R_{\textrm{\textrm{max}}}$, meaning $\xi_{\textrm{min}} = L_{\textrm{X}}/(n_{\textrm{X}} R_{\textrm{\textrm{max}}}^2)$.  Noting that $P_{\textrm{X}} = n_{\textrm{X}} k_{\textrm{B}} T_{\textrm{X}}$ and substituting for $n_{\textrm{X}}$ they re-wrote the new criterion for the onset of thermal sweeping as
< \begin{equation}
< 	\Sigma_{\textrm{\textrm{TS}}}=\sqrt{2\pi}\mu c_c\left(\frac{L_{\textrm{X}} T_{\textrm{X}}}{\Omega \xi_{\textrm{min}} R_{\textrm{\textrm{max}}}^2 T_c}\right)\exp\left(\frac{T_{\textrm{X}}}{2T_c}\right)
< 	\label{newsig1}
< \end{equation}
< which, using standard vales, assuming the dust temperature distribution used in their models and assuming $\xi_{\textrm{min}}=3\times10^{-7}$, is
< %\begin{gather}
< %\nonumber
< %\Sigma_{\textrm{\textrm{TS}}} = 0.14\textrm{g\,cm}^{-2}\left(\frac{L_{\textrm{X}}}{10^{30}\textrm{erg s}^{-1}}\right)%\left(\frac{T_{\textrm{\textrm{1AU}}}}{100\textrm{K}}\right)^{-1/2} \\ \nonumber
< %\times \left(\frac{M_\ast}{0.7M_{\odot}}\right)^{-1/2}\left(\frac{R_{\textrm{\textrm{max}}}}{10\textrm{\textrm{AU}}}\right)^{-1/4} \\ 
< %\times \exp\left[\left(\frac{R_{\textrm{\textrm{max}}}}{10\textrm{\textrm{AU}}}\right)^{1/2} \left(\frac{T_{\textrm{\textrm{1AU}}}}{100\textrm{K}}\right)^{-1} \right]
< %\label{newsig2}
< %\end{gather}
171c174
< \times \left(\frac{M_\ast}{M_{\odot}}\right)^{-1/2}\left(\frac{R_{\textrm{\textrm{max}}}}{\textrm{\textrm{AU}}}\right)^{-1/4} \\ 
---
> \times \left(\frac{M_\ast}{M_{\odot}}\right)^{-1/2}\left(\frac{R_{\textrm{\textrm{max}}}}{\textrm{\textrm{AU}}}\right)^{-1/4} \\
175,176c178,192
< where $L_{\textrm{X}}$, $T_{1\textrm{\textrm{AU}}}$, $R_{\textrm{\textrm{max}}}$ are the X-ray luminosity of the star, the dust temperature at 1\,AU and the radius of maximum surface density (which is assumed to be the inner hole radius). Note that equation \ref{newsig2} in this paper differs from that presented in Owen et al. (2013), which contained mistakes. 
< Although Owen et al. (2013) developed an apparently improved thermal sweeping criterion, they did not investigate the mechanism itself in detail with any multidimensional models
---
> where $L_{\textrm{X}}$, $T_{1\textrm{\textrm{AU}}}$, $R_{\textrm{\textrm{max}}}$ are the X-ray luminosity of the star, the dust temperature at 1\,AU and the radius of maximum surface density (which is assumed to be the inner hole radius).
> 
> 
> The exponential term in the above expression causes the critical
> surface density to increase with radius (see blue line
> in Figure 8); this would imply   
>  an important role for thermal
> sweeping at large radius even for models with relatively high
> surface density normalisation. When this criterion was combined with
> plausible models for disc secular evolution it was predicted that
> thermal sweeping should limit maximum hole sizes in X-ray luminous
> sources to around 25-40 A.U..
> 
> Thermal sweeping is potentially an important mechanism for understanding transition disc populations and planet formation timescales. The critical surface density predictions from Owen et al. (2012, 2013) have already been used in population synthesis 
> simulations by \cite{2015arXiv150904278R}.  However, to date, only two published instances of the instability arising in multidimensional simulations exist. 
178,179d193
< Thermal sweeping is potentially an important mechanism for understanding transition disc populations and planet formation timescales. The critical surface density predictions from Owen et al. (2012, 2013) have already been indirectly imposed in simulations by \cite{2015arXiv150904278R}.  However, to date, only two published instances of the instability arising in multidimensional simulations exist. 
< It is therefore important to test the existing theory of thermal sweeping with new multidimensional simulations.
183c197,202
< rapid clearing is triggered once $\Delta/H$ rises to a value of around unity. 
---
> rapid clearing is triggered once $\Delta/H$ rises to a value of around unity. We find
> that although rapid clearing is indeed associated with large
> $\Delta/H$ values, stable mass loss can still ensue when $\Delta/H$
> is significantly greater than 1. We explore the reason for this difference, 
> develop a new criterion for rapid disc dispersal and discuss the consequences of the new criterion. 
> 
196,223d214
< 
< \section{Numerical Method}
< \label{introBla}
< We perform radiation hydrodynamic (RHD) simulations in this paper using a modified version of the RHD code \textsc{torus} \citep{2000MNRAS.315..722H, 2012MNRAS.420..562H, 2015MNRAS.448.3156H, 2015MNRAS.453.2277H}. \textsc{torus} is primarily a Monte Carlo radiation transport code, though no Monte Carlo radiative transfer is used in this paper. Rather we use the same simplified EUV/X-ray heating prescription of Owen et al. (2012), in part to remain consistent with their work but also to reduce the computational expense. 
< 
< \subsection{Hydrodynamics and gravity}
< \textsc{torus} uses a flux conserving, finite difference hydrodynamics algorithm. It is total variation diminishing (TVD), includes a Rhie-Chow interpolation scheme to prevent odd--even decoupling \citep{1983AIAAJ..21.1525R} and, in this paper, we use the van Leer flux limiter \citep{vanleer}. \textsc{torus} is capable of treating self-gravity using a multigrid method, however in this paper the disc self-gravity is small and so we simply assume a point source potential determined by the star. Testing of the hydrodynamics algorithm in \textsc{torus} is given in \cite{2012MNRAS.420..562H}.
< 
< 
< 
< \subsection{Ionisation parameter heating}
< \label{ionparam}
< We use the scheme implemented by  \cite{2012MNRAS.422.1880O}, where the temperature in any cell optically thin to the X--rays is prescribed as a function of ionisation parameter 
< \begin{equation}
< 	\xi = \frac{L_{\textrm{X}}}{n r^2}
< 	\label{ionparamEq}
< \end{equation}
< where $L_{\textrm{X}}$, $n$ and $r$ are the X-ray luminosity, local number density and distance from the star at which the ionisation parameter is being evaluated. 
< The temperature function $f(\xi)$ was determined by comparison with the Monte Carlo photoionisation code \textsc{mocassin} \citep{2003MNRAS.340.1136E, 2009ApJ...699.1639E} and is given by
< \begin{gather}
< 	T_{\textrm{hot}} = \frac{10^{a_0\log_{10}({\xi})+b_0\log_{10}({\xi})^{-2}}}{1 + c_0\log_{10}({\xi})^{-1} + d_0\log_{10}({\xi})^{-2} + e_0}\\
< 	T_{\textrm{cold}} = \max(10^{f_0\log_{10}({\xi}) + g_0}, T_{\rm{dust}})\\
< 	f(\xi) = \min(T_{\textrm{hot}}, T_{\textrm{cold}})
< 	\label{fxi}
< \end{gather}
< where the numerical constants (subscript 0) are included in Table \ref{constants}. The resulting temperature-ionisation parameter relation is shown in Figure \ref{ionparamplot}. We impose a minimum temperature of 10\,K.  This ionisation parameter heating is applied to all cells that are assumed to be optically thin to the X--rays, which are defined as those from which the column number density to the star is less than $10^{22}$\,cm$^{-2}$ particles \citep{2012MNRAS.422.1880O}. In optically thin cells we consider the maximum of the temperature prescribed by $f(\xi)$ or the dust temperature. In cells optically thick to the X--rays the local dust temperature is applied (see section \ref{discConstruct}).
< 
< 
243a235,244
> \section{Numerical Method}
> \label{introBla}
> We perform radiation hydrodynamic (RHD) simulations in this paper using a modified version of the RHD code \textsc{torus} \citep{2000MNRAS.315..722H, 2012MNRAS.420..562H, 2015MNRAS.448.3156H, 2015MNRAS.453.2277H}. \textsc{torus} is primarily a Monte Carlo radiation transport code, though no Monte Carlo radiative transfer is used in this paper. Rather we use the same simplified EUV/X-ray heating prescription (based on the ionisation parameter in optically thin regions: see 2.2 below) as in  Owen et al. (2012), in part to remain consistent with their work but also to reduce the computational expense. 
> 
> \subsection{Hydrodynamics and gravity}
> \textsc{torus} uses a flux conserving, finite difference hydrodynamics algorithm. It is total variation diminishing (TVD), includes a Rhie-Chow interpolation scheme to prevent odd--even decoupling \citep{1983AIAAJ..21.1525R} and, in this paper, we use the van Leer flux limiter \citep{vanleer}. 
> %\textsc{torus} is capable of treating self-gravity using a multigrid method, however in this paper the disc self-gravity is small and so we simply assume a point source potential determined by the star. 
> Testing of the hydrodynamics algorithm in \textsc{torus} is given in \cite{2012MNRAS.420..562H}.
> 
> 
246,248c247,249
< 	\hspace{-20pt}
< 	\includegraphics[width=9.6cm]{./ionparam2.pdf}
< 	\caption{The temperature-ionisation parameter prescription used for the calculations in this paper. It is constructed using equations 10--12 and the constants in Table 1. The diagonal lines represent lines of constant pressure. }
---
> 	\hspace{-0pt}
> 	\includegraphics[width=9.6cm]{./ionparam.pdf}
> 	\caption{The temperature-ionisation parameter prescription used for the calculations in this paper. It is constructed using equations 10--12 and the constants in Table 1. }
253c254,275
<  %In this work we initially used a temperature dependent step function to specify the mean particle mass for molecular ($\mu=2.33$), atomic ($\mu=1$) and ionised ($\mu=0.5$) gas, however we found that this gave rise to spurious pressure oscillations.  For our published simulations we hence vary the mean particle mass as a smooth ($\tanh$) function of temperature, which is shown in Figure \ref{muOfT}. 
---
> \subsection{Ionisation parameter heating}
> \label{ionparam}
> We use the scheme implemented by  \cite{2012MNRAS.422.1880O}, where the temperature in any cell optically thin to the X--rays is prescribed as a function of ionisation parameter 
> \begin{equation}
> 	\xi = \frac{L_{\textrm{X}}}{n r^2}
> 	\label{ionparamEq}
> \end{equation}
> where $L_{\textrm{X}}$, $n$ and $r$ are the X-ray luminosity, local number density and distance from the star at which the ionisation parameter is being evaluated. 
> The temperature function $f(\xi)$ was determined by comparison with the Monte Carlo photoionisation code \textsc{mocassin} \citep{2003MNRAS.340.1136E, 2009ApJ...699.1639E} and is given by
> \begin{gather}
> 	T_{\textrm{hot}} = \frac{10^{a_0\log_{10}({\xi})+b_0\log_{10}({\xi})^{-2}}}{1 + c_0\log_{10}({\xi})^{-1} + d_0\log_{10}({\xi})^{-2} + e_0}\\
> 	T_{\textrm{cold}} = \max(10^{f_0\log_{10}({\xi}) + g_0}, T_{\rm{dust}})\\
> 	f(\xi) = \min(T_{\textrm{hot}}, T_{\textrm{cold}})
> 	\label{fxi}
> \end{gather}
> where the numerical constants (subscript 0) are included in Table \ref{constants}. The resulting temperature-ionisation parameter relation is shown in Figure \ref{ionparamplot}. We impose a minimum temperature of 10\,K assuming that
> the ambient radiation field sets this florr value.  This ionisation parameter heating is applied to all cells that are optically thin,  defined as those for which the column number density to the star is less than $10^{22}$ particles cm$^{-2}$ \citep{2012MNRAS.422.1880O}. In optically thin cells we set the temperature
> equal to  the maximum of the temperature prescribed by $f(\xi)$ and  the local 
> dust temperature. In cells optically thick to the X-rays the local dust temperature is applied (see section \ref{discConstruct}).
> 
> 
>  %In this work we initially used a temperature dependent step function to specify the mean particle mass for molecular ($\mu=2.33$), atomic ($\mu=1$) and ionised ($\mu=0.5$) gas, but we found that this gave rise to spurious pressure oscillations.  For our published simulations we hence vary the mean particle mass as a smooth ($\tanh$) function of temperature, which is shown in Figure \ref{muOfT}. 
271c293
< We use a 2D cylindrical grid for all models in this paper. Since we assume reflective symmetry about the disc mid plane we only model half of the disc (though we have checked this with simulations that do not assume reflective symmetry, finding any differences are negligible).  \textsc{torus} is capable of using an adaptive or non-uniform mesh, however here we retain the use of a fixed, uniformly spaced, grid to ensure robust results \citep[artificially induced instabilities can possibly arise on non--uniform or adaptive meshes,][]{2000ApJS..131..273F}. Our simulations are MPI parallelized and use domain decomposition. The radiation hydrodynamics works using operator splitting, i.e. we perform hydrodynamic and ionisation parameter heating steps sequentially. We assume a locally isothermal equation of state. We used a variety of total grid sizes and cell numbers, so the resolution varies. However, we always ensured that the disc scale height at the peak surface density radius is resolved by at least 5 cells. We checked for convergence in a test calculation using $128^2$, $256^2$ and $512^2$ cells, finding good agreement, with marginally easier rapid clearing in the lower density simulations. 
---
> We use a 2D cylindrical grid for all models in this paper. Since we assume reflective symmetry about the disc mid plane we only model half of the disc (though we have checked this with simulations that do not assume reflective symmetry, finding any differences are negligible). In this implementation of  \textsc{torus} we use  a fixed, uniformly spaced, grid to ensure robust results \citep[artificially induced instabilities can possibly arise on non--uniform or adaptive meshes,][]{2000ApJS..131..273F}. Our simulations are MPI parallelized and use domain decomposition. The radiation hydrodynamics works using operator splitting, i.e. we perform hydrodynamic and ionisation parameter heating steps sequentially.  We used a variety of total grid sizes and cell numbers, so the resolution varies. However, we always ensured that the disc scale height is resolved by at least 5 cells. We checked for convergence in a test calculation using $128^2$, $256^2$ and $512^2$ cells, finding good agreement, with rapid clearing being marginally easier  in the lowest resolution  simulations. 
273c295,296
< The models are initially allowed to evolve using hydrodynamics only, with the temperature set by the dust temperature only, until the disc is settled. 
---
> The models are initially hydrodynamically evolved without X-ray heating, i.e. with the temperature set by the dust temperature only, until the disc  settles into
> a steady state (typically ? rotation periods at the inner disc rim). 
287c310
< We construct the disc by defining the peak mid plane density $\rho_{\textrm{\textrm{max}}}$ at some radial distance $R_{\textrm{\textrm{max}}}$ (which can be translated into a surface density given the  disc scale height). The mid plane density $\rho_{\textrm{mid}}$ is initially described by
---
> We construct the disc by defining the peak mid plane density $\rho_{\textrm{max}}$ at some radial distance $R_{\textrm{max}}$ (which can be translated into a surface density given the  disc scale height). The mid plane density $\rho_{\textrm{mid}}$ is initially described by
289c312
< 	\rho_{\textrm{mid}} = \rho_{\textrm{\textrm{max}}} (R/R_{\textrm{\textrm{max}}})^{-9/4}.
---
> 	\rho_{\textrm{mid}} = \rho_{\textrm{max}} (R/R_{\textrm{max}})^{-9/4}.
292c315
< The dust temperature distribution is either taken from the models of \cite{2001ApJ...553..321D}, or vertically isothermal and described by
---
> The dust temperature distribution is either taken from the models of \cite{2001ApJ...553..321D}, or is vertically isothermal and described by
294c317
< T_{d} = \max\left({T_{1\rm{\textrm{AU}}}\left(\frac{R}{\rm{\textrm{AU}}}\right)^{-0.5}, 10}\right).
---
> T_{d} = \max\left({T_{1\rm{AU}}\left(\frac{R}{\rm{AU}}\right)^{-0.5}, 10}\right).
297,299c320,324
< Equation \ref{dusttemp} also describes the mid--plane temperature structure well in the D'alessio et al. (2001) models. 
< We use two D'alessio models in this paper, one with $T_{1\textrm{\textrm{AU}}}=50\,$K and one with $T_{1\textrm{\textrm{AU}}}=100$\,K.
< The vertical structure is constructed assuming hydrostatic equilibrium
---
> Equation \ref{dusttemp} also describes the mid--plane temperature structure well in the D'Alessio et al. (2001) models. 
> We use two D'Alessio models in this paper, one with $T_{1\textrm{AU}}=50\,$K and one with $T_{1\textrm{AU}}=100$\,K.
> The vertical structure is initiaaly constructed by imposing
> a profile corresponding to  hydrostatic equilibrium for the case that the
> disc verticaaly isothermal, i.e. 
303c328
< where $H$ is the disc scale height $c_s/\Omega$. For the vertically isothermal models, this gives a surface density profile of the form
---
> where $H$ is the disc scale height $c_s/\Omega$ . This gives a surface density profile of the form
307d331
< The radial surface density profile for the models using the D'alessio et al. (2001) temperature grid is similar, approximately of the form $\Sigma(R)\propto R^{-0.93}$.
309c333,337
< The models in this paper are 2D cylindrically symmetric. We initially impose a Keplerian velocity profile for the azimuthal velocity, the velocity in other directions is initially zero. The radial transition from disc to inner hole is initially not continuous, however we begin the simulation run with hydrodynamics only (i.e. no radiation field) to allow the disc inner edge to relax. Given that these discs are very low mass we use a negligible $\alpha$-viscosity coefficient. 
---
> The models in this paper are 2D cylindrically symmetric. We initially impose a Keplerian velocity profile for the azimuthal velocity while  the velocity in other directions is initially zero. The radial transition from disc to inner hole is initially not continuous, however we begin the simulation run with hydrodynamics only (i.e. no radiation field) to allow the disc inner edge to relax. 
> We set the  $\alpha$-viscosity coefficient to a low value (??)
> as we do not expect secular evolution of the disc due to redistribution
> of angular momentum on the timescale on which the steady state
> wind solution is established. 
312c340
< The properties of the entire disc mid--plane once X--ray photoevaporation begins can also be estimated semi--analytically using an approach which we discuss in the appendix. 
---
> The properties of the entire disc mid--plane can also be estimated semi--analytically using an approach which we discuss in the appendix. 
340,341c368,371
< which was fitted to their simulations results. Being within 40 per cent is perfectly reasonable and comparable to the range of differences between the models and fit from Owen et al. (2012). 
< Furthermore, this factor of 40 per cent is easily accounted for by the uncertainty in defining the surface through which the mass flows on a discrete \textit{cylindrical} grid, compared to the spherical grid used by Owen et al. (2012). 
---
> which was fitted to their simulations results. A deviation of 40 per cent is 
> in line
> with the range of differences between the models and fit from Owen et al. (2012). 
> %Furthermore, this factor of 40 per cent is easily accounted for by the uncertainty in defining the surface through which the mass flows on a discrete \textit{cylindrical} grid, compared to the spherical grid used by Owen et al. (2012). 
343c373
< We also checked that the specific angular momentum and bernoulli constant 
---
> We also checked that the specific angular momentum and Bernoulli constant 
347c377,382
< were invariant along streamlines for a disc in a steady state, finding that these vary by less than 0.035 and 5 per cent along 80AU of streamline respectively. Much of the variation in the Bernoulli constant arises because in order to evaluate the $\int \textrm{d}p/\rho$ term we have to first fit the pressure as a function of $1/\rho$ along the streamline, yielding a simple function of density for this term in the Bernoulli constant. If the flow is not entirely steady a single $1/\rho$ can yield more than one pressure, making the function difficult to fit. 
---
> were invariant along streamlines for a disc in a steady state, finding that these vary by less than 0.035 and 5 per cent along 80AU of streamline respectively. 
> The small variation in the Bernoulli constant arises both from
> the necessity of fitting a barotropic equation of state along
> the streamline in order to evaulate the $\int dp/\rho$  term and from small
> departures from a steady flow.
> %Much of the variation in the Bernoulli constant arises because in order to evaluate the $\int \textrm{d}p/\rho$ term we have to first fit the pressure as a function of $1/\rho$ along the streamline, yielding a simple function of density for this term in the Bernoulli constant. If the flow is not entirely steady a single $1/\rho$ can yield more than one pressure, making the function difficult to fit. 
358,360c393,395
<    $R_{\textrm{\textrm{max}}}$ & 5AU & Inner hole radius\\
<    $\rho_{\textrm{\textrm{max}}}$ & $1\times10^{-14}$g\,cm$^{-3}$ &Peak mid--plane density\\     
<    $T_{\textrm{\textrm{1AU}}}$ & 50\,K & 1AU  mid--plane dust temperature \\
---
>    $R_{\textrm{max}}$ & 5AU & Inner hole radius\\
>    $\rho_{\textrm{max}}$ & $1\times10^{-14}$g\,cm$^{-3}$ &Peak mid--plane density\\     
>    $T_{\textrm{1AU}}$ & 50\,K & 1AU  mid--plane dust temperature \\
364,365c399,400
<    $\Sigma_{\textrm{\textrm{max}}}$ & 0.129\,g\,cm$^{-2}$ & Peak surface density \\
<    $\Sigma_{\textrm{\textrm{TS}}}$ & 0.178\,g\,cm$^{-2}$ & Owen et al. (2012) critical  \\  
---
>    $\Sigma_{\textrm{max}}$ & 0.129\,g\,cm$^{-2}$ & Peak surface density \\
>    $\Sigma_{\textrm{TS}}$ & 0.178\,g\,cm$^{-2}$ & Owen et al. (2012) critical  \\  
381a417,431
> 
> As a further test, we also first consider a thermal sweeping scenario very similar to that in the original calculation presented in Owen et al. (2012). The parameters of this model (which has the same D'Alessio dust temperature structure and has a very similar peak mid--plane density and inner hole radius to the
> original model) 
> are given in Table \ref{model1}. 
> %We note that this simulation is not identical to the original thermal sweeping model, but uses the same D'Alessio dust temperature structure and has a very similar peak mid--plane density and inner hole radius.  
> Snapshots of the density evolution of this first model are given in Figure \ref{xraywarmsnaps}. The morphological evolution is the same as that observed in the original thermal sweeping models. A billowy plume of material at the disc inner edge appears just prior to rapid disc clearing. Once the instability is fully initiated, over 20\,AU of the disc clears in about 700 years. We illustrate the accelerated clearing through 
> Figure \ref{rinnerEvo}: for a surface density profile given by equation (16),
> constant mass loss (as in the case of normal X-ray photoevaporation) results in
> a {\it linear} increase of inner hole radius with time as seen at times less
> than $300$ years. Subsequently, the outward radial velocity increases
> continuouly as the disc undergoes runaway clearing.
> 
> 
>  In summary \textsc{torus} reproduces the behaviour expected from previously published simulations. It conserves physical constants accurately and for stable and unstable discs is consistent with the results presented by Owen et al. (2012). 
> 
384c434
<   \caption{Summary of the parameters of the simulations in this paper. $R_{\textrm{\textrm{max}}}$ is the location of the peak mid--plane density, either in the long-term for a stable disc, or for an unstable disc that just prior to rapid clearing. $\Sigma_{\textrm{\textrm{max}}}$ is the surface density at $R_{\textrm{\textrm{max}}}$.  $T_{1\textrm{\textrm{AU}}}$ is the dust temperature at 1\,AU. $\rho_{\textrm{\textrm{max}}}$ is the mid--plane density at $R_{\textrm{\textrm{max}}}$. All models have $L_{\textrm{X}}=2\times10^{30}$\,erg\,s$^{-1}$.}
---
>   \caption{Summary of the parameters of the simulations in this paper. $R_{\textrm{max}}$ is the location of the peak mid--plane density, either in the long-term for a stable disc, or for an unstable disc that just prior to rapid clearing. $\Sigma_{\textrm{max}}$ is the surface density at $R_{\textrm{max}}$.  $T_{1\textrm{AU}}$ is the dust temperature at 1\,AU. $\rho_{\textrm{max}}$ is the mid--plane density at $R_{\textrm{max}}$. All models have $L_{\textrm{X}}=2\times10^{30}$\,erg\,s$^{-1}$.}
388c438
<    Model ID &  Stellar mass  &    $R_{\textrm{\textrm{max}}}$ & $\Sigma_{\textrm{\textrm{max}}}$ &  $T_{1\textrm{\textrm{AU}}}$ &$\rho_{\textrm{\textrm{max}}}$ & Column & Vertically & Stable?\\
---
>    Model ID &  Stellar mass  &    $R_{\textrm{max}}$ & $\Sigma_{\textrm{max}}$ &  $T_{1\textrm{AU}}$ &$\rho_{\textrm{max}}$ & Column & Vertically & Stable?\\
401c451
< K & 0.1 & 7.7 & $8.7\times10^{-2}$ & 50 & $1.26\times10^{-14}$ & Yes &  Yes & No \\
---
> K & 0.1 & 7.7 & $8.7\times10^{-2}$ & 50 & $1.26\times10^{-14}$ & Yes &  Yes & Yes \\
406,407d455
< P & 0.1 &  25 & 0.1 & 50 & $2.0\times10^{-15}$  &  No & Yes & No \\
< Q & 0.1 &  25 & 1. & 50 & $2.0\times10^{-14}$  &  No & Yes & Yes \\
413,418c461,465
< As a further test, we also first consider a thermal sweeping scenario very similar to that in the original instance presented in Owen et al. (2012). The parameters of this model are given in Table \ref{model1}. We note that this simulation is not identical to the original thermal sweeping model, but uses the same D'alessio dust temperature structure and has a very similar peak mid--plane density and inner hole radius.  Snapshots of the density evolution of this first model are given in Figure \ref{xraywarmsnaps}. The morphological evolution is the same as that observed in the original thermal sweeping models. A billowy plume of material at the disc inner edge appears just prior to rapid disc clearing. Once the instability is fully initiated, over 20\,AU of the disc clears in about 700 years, and in an accelerating fashion (as opposed to the constant rate of change of inner hole radius which is expected for normal, steady, photoevaporation). The evolution of the disc inner hole radius for this model is shown in Figure \ref{rinnerEvo}.
< 
< 
< 
< In summary \textsc{torus} reproduces the behaviour expected from previously published simulations. It conserves physical constants accurately and for stable and unstable discs is consistent with the results presented by Owen et al. (2012). 
< 
---
> \begin{figure}
> 	\includegraphics[width=8.8cm]{./DeltaH.pdf}
> 	\caption{Representative values of $\Delta/H$ for the simulations in this paper. Green and red points are stable and unstable respectively. The blue points are the value of $\Delta/H$ at $R_{\textrm{max}}$ predicted by the semi-analytic tool discussed in the appendix. According to the existing theory, $\Delta/H > 1$ should result in an unstable disc, however these results do not reflect this.}
> 	\label{DeltaH}
> \end{figure}
425c472
< We ran a suite of 2D radiation hydrodynamic simulations of disc photoevaporation, constructed as discussed in section \ref{introBla}. This includes simulations in the column limited and density limited regimes. We explore two stellar mass regimes and a range of disc inner hole radii and masses. All models consider an X--ray luminosity of $2\times10^{30}$\,erg\,s$^{-1}$. A summary of the simulation parameters are given in Table \ref{models}. We run all models until it is clear whether normal clearing or radiative instability is occurring, with a maximum simulation time of about 6000 years. 
---
> We ran a suite of 2D radiation hydrodynamic simulations of disc photoevaporation, constructed as discussed in section \ref{introBla}. These include simulations in the column limited and density limited regimes. We employ  two stellar mass  and a range of disc inner hole radii and masses. All models consider an X--ray luminosity of $2\times10^{30}$\,erg\,s$^{-1}$. A summary of the simulation parameters are given in Table \ref{models}. We run all models until it is clear whether normal clearing or thermal sweeping is occurring, with a maximum simulation time of about 6000 years. 
428d474
< \subsection{Testing the Owen et al. (2013) criterion for the onset of thermal sweeping}
429a476,478
> \subsection{Criterion for the onset of thermal sweeping}
> In the appendix we present a semi--analytic means of estimating the  mid--plane properties of a disc irradiated by X--rays, including the radial variation of $\Delta/H$. Figure \ref{DeltaH} shows the values of $\Delta/H$ at $R_{\textrm{max}}$ for our model discs. The values in the unstable models are measured directly from the simulations. For the stable models, the X--ray heated zone is so small that it is poorly resolved by our simulation, in which case we provide a $\Delta/H$ estimate using the semi-analytic approach discussed in the appendix.
> The values are colour coded, with blue triangles and red crosses being stable and unstable respectively. Although every unstable model does have $\Delta/H > 1$, there are simulations (J and K) with $\Delta/H$ expected to be $>1$ which are stable. Furthermore, there are some stable discs with higher predicted $\Delta/H$ than unstable discs (e.g. compare model K with  H and L). Clearly then, $\Delta/H > 1$ is not is not the exclusive criterion for rapid radiative disc dispersal. We note that once instability does initiate, $\Delta/H$ measured directly in the simulations is greater than unity, but also fluctuates significantly, making it difficult to prescribe a directly measured value of the ratio. 
431,434d479
< In Figure \ref{sigma13} we show the ratio of the peak disc surface density in our models to the surface density at which thermal sweeping is predicted to initiate according to the Owen et al. (2013) approach (equation \ref{newsig2} in this paper). The points are colour coded blue and red for stable and unstable models respectively. An accurate criterion should separate the stable and unstable models about a ratio value of 1. The Owen et al. (2013) approach predicts that all models except model A should be unstable, however this is certainly not the case in the simulations. 
<  There is some deficiency in the approach used to determine the thermal sweeping criterion by Owen et al. (2013) that was not realised because they ran no 2D radiation hydrodynamic simulations that followed the instability, rather just used 1D models and tracked the expected value of $\Delta/H$.
< 
< In the appendix, we present a means of estimating the properties of an X--ray irradiated disc, including estimating $\Delta/H$. In Figure  \ref{DeltaH} we plot the analytic values of $\Delta/H$ for the simulations. Again, the values are colour coded, with blue  and red points being stable and unstable respectively. There are both unstable models with $\Delta/H<1$ and a stable model with $\Delta/H>1$ so, again, our results imply that $\Delta/H=1$ is not the fundamental criterion for instability. Note, however, that once instability does initiate in a simulation we do find that $\Delta/H>1$.
439,441d483
< 
< 
< 
443,446c485,487
< 	\hspace{-15pt}
< 	\includegraphics[width=8.8cm]{./Owen13sigma.pdf}
< 	\caption{The ratio of the model peak surface density to the critical surface density for thermal sweeping according to the Owen et al. (2013) approach - equation 8 in this paper. Stable and unstable models should be separated by a ratio value of unity.}
< 	\label{sigma13}
---
> 	\includegraphics[width=8.8cm]{./Interior_new2.pdf}
> 	\caption{The mid--plane density profile of disc inner edges alongside the density profile below which gas is heated above the local dust temperature ($\rho_{\textrm{heat}}$). The column to which the gas is optically thick to the X--rays is illustrated by the blue arrows. For the red solid line, which has gas above the critical density, X--rays cannot heat the gas above the dust temperature once they reach the point of intersection with $\rho_{\textrm{heat}}$. For the green dashed line, the gas is always heated above the dust temperature and so perturbations causing the X--rays to penetrate further into the disc always result in further heating and hence further perturbation.}
> 	\label{interior}
450d490
< 
452,455c492,494
< 	\hspace{-15pt}
< 	\includegraphics[width=8.8cm]{./DeltaH.pdf}
< 	\caption{Representative values of $\Delta/H$ for the simulations in this paper. Green and red points are stable and unstable respectively. The blue points are the value of $\Delta/H$ at $R_{\textrm{\textrm{max}}}$ predicted by the semi-analytic tool discussed in the appendix. According to the existing theory, $\Delta/H > 1$ should result in an unstable disc, however these results do not reflect this.}
< 	\label{DeltaH}
---
> 	\includegraphics[width=8.8cm]{./schematic_TS2.pdf}
> 	\caption{A schematic showing why rapid disc dispersal is suppressed if densities at the disc inner edge are sufficiently high that the gas is not heated above the local dust temperature. Compare with Figure \ref{schemTSWarm}.}
> 	\label{schemTSCold}
457a497,501
> \begin{figure}
> 	\includegraphics[width=8.8cm]{./rhoMax.pdf}
> 	\caption{The ratio of the disc maximum volume density to the critical maximum volume density for rapid radiative disc dispersal (equation \ref{criticalRho}). There is a clear transition from instability to stability once the ratio exceeds unity.}
> 	\label{rhoMax}
> \end{figure}
461,464c505,508
< 	\hspace{-15pt}
< 	\includegraphics[width=8.8cm]{./IonParamCriterion.pdf}
< 	\caption{The ratio of the disc maximum mid--plane pressure to the critical pressure  for rapid radiative disc dispersal (equation \ref{pcrit}). There is a clear transition from instability to stability once the ratio exceeds unity.}
< 	\label{ionparamcrit}
---
> 	\hspace{-10pt}
> 	\includegraphics[width=9cm]{./comparison.pdf}
> 	\caption{A comparison of the critical surface density for thermal sweeping from Owen et al. (2012, 2013) and the new relation derived here. Note that the new relation only applies to a vertically isothermal disc and will likely be a lower limit for warmer discs with lower mid--plane densities. This plot assumes $T_{\textrm{X}}=400$\,K, $T_{\textrm{1AU}}=100$\,K and $M_*= 0.7\,M_{\odot}$. The black line shows the $R^{-1}$ radial variation of the surface density profile implemented in our simulations. }
> 	\label{compare}
467a512
> We do find an alternative and very simple criterion for thermal sweeping which applies in both the column limited and density limited regimes, which is that clearing always happens when the maximum mid--plane density in the disc drops to a sufficiently low value that it would be elevated above the local dust temperature if optically thin to the X--rays. 
469,470c514,561
< \subsection{A new criterion for thermal sweeping}
< We do find an alternative criterion for thermal sweeping. Consider Figure \ref{ionparamplot}; isobars are traced diagonally across this plot, such that the maximum possible pressure is the feature at an ionisation parameter of $\sim 1\times10^{-7}$. In the regime between the pressure maximum and the floor temperature of 10\,K, a drop in the density would imply an increase in ionisation parameter, temperature \textit{and pressure} (since the temperature--ionisation parameter relation is steeper than the isobars in this regime). The increase in pressure would hence lead to further perturbation. If the pressure maximum from the temperature--ionisation parameter relation is larger than the maximum pressure in the disc mid--plane, then the disc will never be able to support against the X--ray heated gas and the perturbation will be able to proceed throughout the entire disc. 
---
> %Once the peak mid--plane density in the disc can be heated above the dust temperature \textit{all of the disc inner edge optically thin to the X--rays can be heated above the local dust temperature}. 
>  We provide a schematic illustration in  Figure \ref{interior} of why
> this criterion is fundamental to the onset of runway clearing.
> The red and green curves denote the density profiles of the dust heated disc for
> two different density normalisations: the fall-off at the disc edge inward of
> the maximum is
> described by a Gaussian in radius with scale length equal to the vertical
> scale height (Owen et al 2013) while the profile outward of the maximum
> is the power law profile (equation \ref{rhodist}. The dashed line represents the density at each radius at which the temperature of X-ray heated gas would equal
> the dust temperature. In the 
> left hand panel, the extent of the X-ray heated region is density
> limited and the location of the X-ray heated interface is set by the
> intersection of this line with the disc density profile, i.e. point X
> in the case of the higher density normalisation. In the case of the
> lower density normalisation there are evidently no
> intersections and runawat clearing is expected. The right hand panel
> is a schematic depiction of the case where the X-ray heated region is
> column limited, located at points Y and Z in each case. Whereas these
> are equilibrium points they are not necessarily stable. In the case
> that there is a perturbation in the X-ray heated column (e.g. mass
> loss perpendicular to the disc plane) then the X-rays will heat further
> into the disc. For the case with higher density normalisation, this
> incursion into the disc cannot proceed firther than point X because,
> even under optically thin conditions, the X-rays cannot heat gas at this
> density above the local dust temperature. In the case of the lower
> density normalisation, such an incursion of X-ray heating into
> the disc is not limited by the existence of a stable equilibrium
> in the density limited regime and runaway clearing would
> occur. We thus expect that the criterion for thermal sweeping involves
> a comparison of the maximum mid-plane density in the disc with the critical
> density.    
> %Tbe radial dependence of the critical density
> %below which the X-ray heated temperature exceeds the dust temperature is
> $shown by the dashed line. , which shows the density profile at the disc inner edge (assuming it is similar to the vertical structure at $R_{\textrm{max}}$) as well as the density below which X--rays can heat the gas $\rho_{\textrm{heat}}$. When the criterion is satisfied, perturbations at the disc inner edge allow the optically thin column to propagate \textit{and heat} further into the disc towards the peak density and beyond. If the peak density is higher than the critical value, then at some point interior to the radius of peak density the column of gas optically thin to the X--rays will become density limited. This means that although perturbations at the disc inner edge will allow the optically think column to penetrate further into the disc \textit{there will be no further heating and hence no runaway clearing}. A schematic of the behaviour when the peak mid--plane density is above the critical value (will not be heated above the dust temperature if optically thin) is given in Figure \ref{schemTSCold}, which compared with Figure \ref{schemTSWarm} illustrates why clearing is suppressed.
> 
> 
> Quantitatively, we evaluate the critical density by noting from Figure 2 that
> there is a  rapid decline in the temperature of X-ray heated gas at low
> ionisation parameter ($\xi_{\rm min}$) and we can thus use equation
> \ref{ionparamEq} to obtain:
> i%inradiative clearing occurs if the peak mid--plane volume density at radius $R_{\textrm{max}}$, $\rho_{\textrm{max}}$ is less than $\rho_{\textrm{TS}}$, where the latter stems from equation \ref{ionparamEq} and is given by
> \begin{equation}
> 	\rho_{\textrm{TS}} = \frac{\mu m_{\textrm{H}} L_{\textrm{X}}}{\xi_{\textrm{min}}R_{\textrm{max}}^2}.
> 	\label{criticalRho}
> \end{equation}
> where $R_{\textrm{max}}$ is the radius of the disc inner edge (i.e. the
> location of the density maximum in the disc). 
> We plot the ratio of the disc maximum density to that given by equation \ref{criticalRho} in Figure \ref{rhoMax}. We assume a value of $\xi_{\textrm{min}} = 3\times10^{-8}$, which we find is typical of discs when using the semi-analytic approach to determining the mid-plane properties that we present in the appendix. There is a clear transition from stability to instability once the peak mid--plane density in the disc drops below the critical value given by equation \ref{criticalRho}. 
472,482c563,565
< Quantitatively, instability will occur when the maximum mid--plane pressure in the disc $P_{\textrm{max}}$ is less than the pressure maximum from the temperature--ionisation parameter relationship 
< \begin{equation}
< 	P_{\textrm{crit}} = \frac{L_{\textrm{X}}}{\xi_{\textrm{crit}}R_{\textrm{max}}^2}k_B T_{\textrm{crit}}.
< 	\label{pcrit}
< \end{equation}
< From the temperature--ionisation parameter relation, we find that $\xi_{\textrm{crit}}=1.2\times10^{-7}$ and $T_{\textrm{crit}}=113\,$K. In Figure \ref{ionparamcrit} we plot the ratio of the peak disc mid--plane temperature to the critical pressure (equation \ref{pcrit}), which shows that our new criterion does clearly separate the stable and unstable models about a pressure ratio of unity and is therefore correct. Equating the critical pressure to the maximum in the disc, we find that the critical peak mid--plane volume density for thermal sweeping is
< \begin{equation}
< 	n_{\textrm{TS}} = 4.2\times10^{10}\left(\frac{R_{\textrm{max}}}{\textrm{AU}}\right)^{-3/2}\left(\frac{T_{\textrm{1AU}}}{100}\right)^{-1}\left(\frac{L_{\textrm{X}}}{10^{30}}\right).
< 	\label{nts}
< \end{equation}
< Although we go on to discuss critical surface densities, it is important to emphasise that under this new description, thermal sweeping is actually determined by a criterion on the volume density, not the surface density. One could therefore conceive of two discs with identical surface densities, but different thermal structures such that the mid--plane density differs sufficiently that one disc is stable and the other unstable. Nevertheless, in practice a surface density criterion for thermal sweeping is more accessible and more useful than a volume density estimate. According to our simulations, a vertically isothermal disc has a higher mid-plane density than simulations using the D'alessio temperature grid. Assuming a vertically isothermal disc to calculate the critical surface density for thermal sweeping should therefore provide a reasonable lower limit, hence
---
> 
> 
> It is important to emphasise that thermal sweeping is actually determined by a criterion on the volume density, not the surface density. One could therefore conceive of two discs with identical surface densities, but different thermal structures such that the mid--plane density differs sufficiently that one disc is stable and the other unstable. Nevertheless, in practice a surface density criterion for thermal sweeping is more accessible and more useful than a volume density estimate. According to our simulations, a vertically isothermal disc has a higher mid-plane density than simulations using the D'alessio temperature grid. Assuming a vertically isothermal disc to calculate the critical surface density for thermal sweeping should therefore provide a reasonable lower limit, hence
484c567
< 	\Sigma_{\textrm{\textrm{TS}}} \approx \rho_{\textrm{\textrm{TS}}}\frac{c_s}{\Omega}
---
> 	\Sigma_{\textrm{TS}} \approx \rho_{\textrm{TS}}\frac{c_s}{\Omega}
486c569
< which, using equation \ref{nts}, assuming $\mu = 1.37125$ and inserting other constants, results in
---
> which, using equation 9, assuming $\mu = 1.37125$, $\xi_{\textrm{min}}=3\times10^{-8}$ and inserting other constants, results in
488c571,572
< 	\Sigma_{\textrm{\textrm{TS}}} = 0.037547\textrm{\,g\,cm}^{-2}\left(\frac{L_{\textrm{X}}}{10^{30}}\right)\left(\frac{M_*}{M_{\odot}}\right)^{-1/2} \\ \times \left(\frac{T_{\textrm{1AU}}}{100}\right)^{-1/2}\left(\frac{R_{\textrm{max}}}{\textrm{AU}}\right)^{-1/4}.
---
> 	\Sigma_{\textrm{TS}} \approx 0.0237\,\textrm{g}\,\textrm{cm}^{-2} \left(\frac{L_{\textrm{X}}}{10^{30}\textrm{erg s}^{-1}}\right)\left(\frac{T_{\textrm{1AU}}}{100\,\textrm{K}}\right)^{1/2} \\
> 	\times \left(\frac{M_*}{M_{\odot}}\right)^{-1/2}\left(\frac{R_{\textrm{max}}}{10\,\textrm{AU}}\right)^{-3/4}. 
491,501c575
< Which, interestingly, is almost identical to the expression derived using the Owen et al. (2013) approach, only without the exponential term. Note that this relation is not strictly correct at all radii, since it assumes that the temperature always scales as $R^{-1/2}$ with no floor value. For the simulations in this paper, beyond a radius of 
< \begin{equation}
< 	R_{floor} = 1\,\textrm{\textrm{AU}}\left(\frac{T_{\textrm{1AU}}}{10}\right)^2
< \end{equation}
< the radial temperature will be isothermal at 10\,K and the critical surface density for thermal sweeping is 
< \begin{equation}
< 	\Sigma_{\textrm{TS}} = 0.1187\textrm{\,g\,cm}^{-2}\left(\frac{L_{\textrm{X}}}{10^{30}}\right)\left(\frac{M_*}{M_{\odot}}\right)^{-1/2}\left(\frac{R_{\textrm{max}}}{\textrm{AU}}\right)^{-1/2}
< 	\label{myTSequn2}
< \end{equation}
< 
< 
---
> We compare this new relation alongside the Owen et al. (2012) and Owen et al. (2013) expressions in Figure \ref{compare}. In constructing Figure \ref{compare} we assume that $T_{\textrm{X}}=400$\,K, $T_{\textrm{1AU}}=100$\,K and $M_*= 0.7\,M_{\odot}$ (in addition to vertical isothermality). The behaviour of the new condition is qualitatively very different, with the critical surface density being more readily attained at smaller inner hole radii (less than about 1\,AU) but being much more difficult to attain at radii beyond a few AU. It is important to note that the radial decrease of the disc surface density in our models is \textit{steeper} than the radial decrease in the peak surface density. A disc becoming unstable to rapid radiative clearing  at small radii should hence clear out the whole disc. 
505c579,599
< We compare this new composite relation (equations \ref{myTSequn}, \ref{myTSequn2}) alongside the Owen et al. (2012) and Owen et al. (2013) expressions in Figure \ref{compare}. In constructing Figure \ref{compare} we assume that $T_{\textrm{X}}=400$\,K, $T_{\textrm{\textrm{1AU}}}=50$\,K and $M_*= 0.1\,M_{\odot}$ (in addition to vertical isothermality). The behaviour of the new condition is qualitatively very different, being much more difficult to attain the critical surface density at radii beyond a few AU. It is important to note that the radial decrease of the disc surface density in our simulations is \textit{steeper} ($\Sigma \propto R^{-1}$) than the radial decrease in the critical surface density ($\Sigma \propto R^{-1/4}$ or $\Sigma \propto R^{-1/2}$). A disc becoming unstable to rapid radiative clearing  at small radii should hence clear out the whole disc. 
---
> %\begin{table*}
> % \centering
> %  \caption{Summary of the parameters of the simulations in this paper. }
> %  \label{models}
> %  \begin{tabular}{@{}l l l l l l l l c l@{}}
> %  \hline
> %   Model ID &  Stellar mass  & Initial disc mass & X-ray luminosity& Hole radius & $\Sigma_{\textrm{max}}$ & $%\Sigma_{\textrm{max}}/\Sigma_{\textrm{TS}}$ & $T_{1\textrm{au}}$ &$\rho_{\textrm{max}}$ & Regime\\
>  % &  M$_\odot$ &M$_\odot$ &  $10^{30}$erg/s& AU & g\,cm$^{-2}$ & & K & g\,cm$^{-3}$\\
>  %\hline
>  %A & 0.1 & & 2 & 5 & & & 50 &  & X-ray warm \\
>  %B & 0.1 & & 2 & 10 & & & 50 & &X-ray warm \\ 
>  %C & 0.7 & & 2 & 10 & & & 50 & &X-ray warm \\ 
>  %D & 0.7 & & 2 & 20 & & & 50 & &X-ray cold \\ 
>  %E & 0.7 & & 2 & 30 & & & 50 & &X-ray cold \\ 
>  %F & 0.7 & & 2 & 30 & & & 50 & &X-ray cold \\ 
>  %G & 0.7 & & 2 & 30 & & & 50 & &X-ray cold \\  
>  %H & 0.7 & & 2 & 30 & & & 50 & &X-ray cold \\   
>  %Test & 0.1 & $4.85\times10^{-3}$ & 2 & 7.2 &4.71 &33.64 & 50 & &X-ray warm \\  
> %\hline
> %\end{tabular}
> %\end{table*}
507d600
< We reiterate that the actual criterion is on the peak mid--plane pressure and hence the volume density, not the surface density. We should therefore not expect the new surface density criterion to be be completely accurate. In Figure \ref{sigma2} we show the ratio of the model peak surface density to the critical surface density for thermal sweeping given by our new criterion. Compared with the old criterion (see Figure \ref{sigma13}) there is much better agreement, the new solution is accurate to within a factor of 2, despite the surface density not being the fundamental parameter.
509,514d601
< \begin{figure}
< 	\hspace{-10pt}
< 	\includegraphics[width=9cm]{./comparison_0p1Msol_10Kfloor.pdf}
< 	\caption{A comparison of the critical surface density for thermal sweeping from Owen et al. (2012, 2013) and the new relation derived here. Note that the new relation only applies to a vertically isothermal disc and will likely be a lower limit for warmer discs with lower mid--plane densities. This plot assumes $T_{\textrm{X}}=400$\,K, $T_{\textrm{\textrm{1AU}}}=50$\,K and $M_*= 0.1\,M_{\odot}$. }
< 	\label{compare}
< \end{figure}
518,524d604
< \begin{figure}
< 	\hspace{-10pt}
< 	\includegraphics[width=9cm]{./newApproachSigma.pdf}
< 	\caption{The ratio of the model peak surface density to the critical surface density for thermal sweeping according to our new criterion - equation 22 in this paper. Stable and unstable models should be separated by a ratio value of unity. The new criterion is much more accurate than the old (see Figure \ref{sigma13}). Note that the new criterion is formally on the volume density, not the surface density, which may explain the small discrepancies.}
< 	\label{sigma2}
< \end{figure}
< 
530,531d609
< 
< 
533,534c611,612
< Combining the theory of normal disc photoevaporation detailed by Owen et al. (2010, 2011, 2012) with the theory of viscous disc accretion presented by \cite{1998ApJ...495..385H} we can constrain
< the maximum possible inner hole radius for viscous discs with inner holes opened by photoevaporation. For normal photoevaporation the photoevaporative mass loss rate  
---
> Using the theory of normal disc photoevaporation detailed by Owen et al. (2010, 2011, 2012) we can constrain
> the maximum possible inner hole radius for discs with inner holes opened by photoevaporation. For normal photoevaporation the photoevaporative mass loss rate  
539c617
< is approximately equal to the accretion rate. Using the form of a viscous accretion disc given by \cite{1998ApJ...495..385H}, at the time of gap opening the surface density profile is
---
> is approximately equal to the accretion rate
541,542c619
< 	\Sigma_{GO} = \frac{M_d(0)}{2\pi RR_1}T_{GO}^{-3/2}\exp\left(-\frac{R}{R_1T_{GO}}\right)
< 	\label{Hartmann}
---
> 	\dot{M}_{acc} = \frac{3\pi \alpha c_s^2\Sigma_G}{\Omega}
544c621
< where the time of gap opening in the disc by photoevaporation is given by 
---
> where $\Sigma_G$ is the surface density at the gap inner edge and $\alpha$ is the viscosity parameter.  Assuming an $R^{-1}$ surface density profile  until the exponential decrease in density at the disc outer edge, the surface density at any radius $R$ in such a disc is 
546c623,624
< 	T_{GO} = \left(\frac{M_d(0)}{2t_s\dot{M_w}}\right)^{2/3}.
---
> \Sigma(R) = \Sigma_G(R/R_G)^{-1}\exp(-R/R_1)
> \label{sigmaRexp}
548c626
< Equating equation \ref{Hartmann} to the thermal sweeping criterion (equation \ref{myTSequn}) we can solve for the radius at which thermal sweeping will initiate for a viscous accretion disc undergoing photoevaporation. Unfortunately the exponential term is always important, requiring the clearing radius to be solved numerically, that is, finding the value of $R$ for which 
---
> where $R_1$ controls the radius at which the exponential falloff in density becomes effective. Equating equations \ref{sigmaRexp} and \ref{myTSequn}, rapid clearing thus happens when 
550,552c628
< 	1.77\left(\frac{R}{AU}\right)^{-1}\frac{1}{\alpha}\left(\frac{M_*}{M_{\odot}}\right)^{1/2}\left(\frac{T_{1au}}{100}\right)^{-1}\\ \times \exp\biggr(2.5\times10^{-3}\left(\frac{R}{AU}\right)\left(\frac{M_d(0)}{10^{-2}M_{\odot}}\right)^{-2/3}\left(\frac{L_X}{10^{30}}\right)^{2/3} \\
< 	\times \alpha^{-2/3}\left(\frac{T_{1au}}{100}\right)^{-2/3}\left(\frac{R}{AU}\right)^{-1/3} \left(\frac{M_*}{M_{\odot}}\right)^{1/3}\biggr) \\
< 	= 0.037547\textrm{\,g\,cm}^{-2}\left(\frac{M_*}{M_{\odot}}\right)^{-1/2} \left(\frac{T_{\textrm{1AU}}}{100}\right)^{-1/2}\left(\frac{R}{\textrm{AU}}\right)^{-1/4}.
---
> 	\frac{26125}{\alpha}R_G^{-A}\left(\frac{M_*}{M_{\odot}}\right)\left(\frac{T_{1AU}}{100\,K}\right)^{-3/2} \leq R^{(1/4-A)}\exp(R/R_1)
554,555c630,631
< is satisfied. In Figure \ref{rinner_plot} we plot the full numerically evaluated solution. We assume that $R_1$ is 0.6 times the disc outer radius \citep{1998ApJ...495..385H}, that the disc outer radius (which sets $R_1$) varies  from 200 to 400\,AU quadratically with the stellar mass and that the disc mass is 1 per cent of the stellar.  We scale the X--ray luminosity from $10^{29}$ to $10^{30}$\,erg\,s$^{-1}$ from 0.1 to 0.7\,M$_{\odot}$ based on the observations of \cite{2005ApJS..160..401P}. 
< We also assume that $T_{1\textrm{\textrm{AU}}}$ scales linearly in accordance with the values used for the simulations in this paper (i.e. 50 and 100\,K for 0.1 and 0.7\,M$_{\odot}$ stars respectively). For discs evolving normally under the action of viscous accretion and photoevaporation, it appears that thermal sweeping will not clear the disc out to very large radii except at the very lowest masses. It is important to note that this assumes that only the disc inner edge evolves after the time of gap opening.
---
> which has to be evaluated numerically. We plot this radius as a function of mass in Figure \ref{rinner_plot}.  To construct this plot we assume that $T_{1\textrm{AU}}$ scales linearly in accordance with the values used for the simulations in this paper.  We also assume that $(R_G/AU)\approx 3(M_*/M_{\odot})$ and a constant $R_1=300\,$AU. This plot implies that, under the assumptions made here, for most discs with inner holes opened by photoevaporation rapid radiative clearing cannot happen out to very large radii in the disc. This implies that, except for very low mass stars, thermal sweeping will only initiate in components of the disc close to the outer radius, where the density decreases exponentially.  
> 
557,558c633
< 	\hspace{-15pt}
< 	\includegraphics[width=9cm]{./exponential.pdf}
---
> 	\includegraphics[width=9cm]{./TS_radius.pdf}
563,587c638
< 
< That rapid clearing should not realistically initiate for photo evaporating viscous discs might seem surprising given the range of unstable models presented here. This is because these models have all been manually constructed without any consideration of the photoevaporation history of the disc, so have surface densities lower than would be expected for a disc evolving under viscous accretion and photoevaporation alone. 
< 
< \begin{figure*}
< 	\includegraphics[width=17cm]{./hist.pdf}
< 	\caption{Histograms showing the ratio of the non-accreting to accreting transition disc lifetimes (left panel) and inner hole radii at which thermal sweeping initiates (right panel). For a population of discs evolving under the combined action of viscosity, X-ray photoevaporation and the new thermal sweeping criterion given in Equation \ref{myTSequn}. }
< 	\label{histograms}
< \end{figure*}
< 
< 
< 
< %Unfortunately this needs to be solved numerically since radial terms are retained both interior and exterior to the exponential term. In order to solve for the radius numerically, a disc mass, outer disc radius, viscosity parameter ($\alpha$), stellar mass, X--ray luminosity and dust temperature at 1\,AU are required. 
< 
< %Although this clearing radius generally needs to be solved numerically, a cleaner solution is available in the limit that the exponential term becomes negligible. In this case the disc surface density at gap opening is
< %\begin{multline}
< %	\Sigma_{GO}(R) = 1.78\frac{1}{\alpha}\left(\frac{L_{\textrm{X}}}{10^{30}}\right) \left(\frac{T_{\textrm{1AU}}}{100}\right)^{-1}\left(\frac{M_*}{M_{\odot}}\right)^{1/2} \\
< %	\times \left(\frac{R_1}{\textrm{AU}}\right)\left(\frac{R}{\textrm{AU}}\right)^{-2}
< %\end{multline}
< %which equated to the critical surface density for thermal sweeping gives a clearing radius of 
< %\begin{multline}
< %	\left(\frac{R_{\textrm{TS}}}{\textrm{AU}}\right) = 6.885\left(\frac{1}{\alpha}\right)\left(\frac{M_*}{M_{\odot}}\right) \\ \times \left(\frac{T_{\textrm{1AU}}}{100}\right)^{-1/2}\left(\frac{R_1}{\textrm{AU}}\right)\left(\frac{R_{\textrm{max}}}{\textrm{AU}}\right).
< %\end{multline}
< 
< 
< 
---
> The difficulty in rapidly clearing the disc might seem surprising given the thermal sweeping calculation of Owen et al. (2012) and the range of unstable models presented here. However these models have all been manually constructed without any consideration of the photoevaporation history of the disc. For example the original thermal sweeping model has a surface density profile three orders of magnitude lower than that given by equation \ref{sigmaRexp}. Under the description of thermal sweeping given by Owen et al. (2013), the exponential dependence of the thermal sweeping criterion on radius (see equation \ref{newsig2}) did lead to rapid clearing at intermediate radii in normal discs. However in our new, tested, model of rapid radiative clearing there is no such dependence, rather rapid clearing is more difficult to initiate at larger radii. 
591c642
< %	\Sigma(R) = f\frac{0.177}{\alpha}\left(\frac{M_*}{M_{\odot}}\right)^{1/2}\left(\frac{T_{\textrm{\textrm{1AU}}}}{100}\right)^{-1}\left(\frac{L_{\textrm{X}}}{10^{30}}\right)\left(\frac{R}{\textrm{10\,AU}}\right)^{-1}
---
> %	\Sigma(R) = f\frac{0.177}{\alpha}\left(\frac{M_*}{M_{\odot}}\right)^{1/2}\left(\frac{T_{\textrm{1AU}}}{100}\right)^{-1}\left(\frac{L_{\textrm{X}}}{10^{30}}\right)\left(\frac{R}{\textrm{10\,AU}}\right)^{-1}
597c648
< %	\left(\frac{R}{10\textrm{\textrm{AU}}}\right) = f\frac{7.47}{\alpha}\left(\frac{M_*}{M_{\odot}}\right)\left(\frac{T_{1\textrm{\textrm{AU}}}}{100}\right)^{-3/2}\left(\frac{R_{\textrm{\textrm{max}}}}{10\textrm{\textrm{AU}}}\right)^{3/4}. 
---
> %	\left(\frac{R}{10\textrm{AU}}\right) = f\frac{7.47}{\alpha}\left(\frac{M_*}{M_{\odot}}\right)\left(\frac{T_{1\textrm{AU}}}{100}\right)^{-3/2}\left(\frac{R_{\textrm{max}}}{10\textrm{AU}}\right)^{3/4}. 
600c651
< %	\left(\frac{R}{10\textrm{\textrm{AU}}}\right) = \left[\frac{7.468 f}{\alpha} \left(\frac{T_{1\textrm{\textrm{AU}}}}{100}\right)^{-3/2} \left(\frac{M_*}{M_{\odot}}\right) \right]^4
---
> %	\left(\frac{R}{10\textrm{AU}}\right) = \left[\frac{7.468 f}{\alpha} \left(\frac{T_{1\textrm{AU}}}{100}\right)^{-3/2} \left(\frac{M_*}{M_{\odot}}\right) \right]^4
611a663,668
> \begin{figure*}
> 	\includegraphics[width=17cm]{./hist.pdf}
> 	\caption{Histograms showing the ratio of the non-accreting to accreting transition disc lifetimes (left panel) and inner hole radii at which thermal sweeping initiates (right panel). For a population of discs evolving under the combined action of viscosity, X-ray photoevaporation and the new thermal sweeping criterion given in Equation \ref{myTSequn}. }
> 	\label{histograms}
> \end{figure*}
> 
619c676
< Since our new calculations have suggested the Owen et al. (2013) thermal sweeping criterion is an overestimate then it is important to quantify the effect a much less efficient thermal sweeping process would have on a population of evolving discs. Owen et al. (2012, 2013) suggested that thermal sweeping would destroy the outer disc almost immediately after photoevaporation had opened a gap in the inner disc and it had drained onto the central star. Such a rapid destruction was necessary to avoid producing a large number of non-accreting transition discs with large holes.
---
> Since our new calculations have suggested the Owen et al. (2013) thermal sweeping criterion is probably an overestimate then it is important to quantify the effect a much less efficient thermal sweeping process would have on a population of evolving discs. Owen et al. (2012,2013) suggested that thermal sweeping would destroy the outer disc almost immediately after photoevaporation had opened a gap in the inner disc and it had drained onto the central star. Such a rapid destruction was necessary to avoid producing a large number of non-accreting transition discs with large holes.
621c678
< With this much less efficient thermal sweeping process we must now quantify how long it takes to destroy the outer disc after photoevaporation has begun to clear the disc and the properties of the transition disc population created during disc dispersal with photoevaporation and thermal sweeping.
---
> With this much less efficient thermal sweeping process we must now quantify how long it takes to destroy the outer disc after photoevaporation has begun to clear the disc and the properties of the transition disc population created during disc dispersal with photoevapo- ration and thermal sweeping.
624c681
< After the gap has opened and the inner disc has drained we assume thermal sweeping takes place once the peak surface density in the remaining outer disc drops below the threshold given in Equation \ref{myTSequn}. We then record the inner hole radius where this occurred, remaining disc mass and the time-scales the disc would have appeared as a accreting and non-accreting transition disc.
---
> After the gap has opened and the inner disc has drained we assume thermal sweeping to place once the peak surface density in the remaining outer disc drops below the threshold given in Equation \ref{myTSequn}. We then record the inner hole radius where this occurred, remaining disc mass and the time-scales the disc would have appeared as a accreting and non-accreting transition disc.
633,634c690
< \noindent 1) Rapid radiative clearing does not fundamentally occur when the ratio of vertical and radial pressure scale lengths $\Delta/H = 1$, as proposed by Owen et al. (2012, 2013). Rather, it depends upon the fact that perturbations that reduce the density in the X--ray heated gas at the disc inner edge lead to an increase in the gas temperature and pressure, which leads to further perturbation. This will continue until the maximum X--ray heated pressure is obtained and will clear through the disc up until the point that the maximum X--ray heated pressure is less than the dust heated pressure. Hence, if the peak possible X--ray heated pressure exceeds the peak mid--plane dust heated disc pressure, the entire disc will eventually be dispersed 
< following perturbation. Note, that this new criterion is specifically on the volume density, not the surface density. Although $\Delta/H$ is not the fundamental criterion, this ratio is still much larger than unity once a disc becomes unstable. \\
---
> \noindent 1) Rapid radiative clearing does not fundamentally occur when the ratio of vertical and radial pressure scale lengths $\Delta/H = 1$, as proposed by Owen et al. (2012, 2013). Rather, it occurs when the peak mid--plane \textit{volume density} in the disc is sufficiently low that it would be heated above the local dust temperature if optically thin to the X--rays. When this happens, all gas at the disc inner edge optically thin to the X--rays is heated above the local dust temperature. Hence perturbations at the disc inner edge allows X--rays to penetrate \textit{and heat} further into the disc, right up to the density maximum and beyond. When the maximum cannot be heated above the dust temperature by X--rays, the X--rays will eventually encounter gas that they cannot heat and the disc will be stable against perturbations. Although $\Delta/H$ is not the fundamental criterion, this ratio is still much larger than unity in our simulations of unstable discs, providing the perturbation. \\
638c694
< \noindent 3) We use the previously established theory of disc photoevaporation to calculate the maximum possible inner hole radius as a function of the stellar mass, for discs with gaps opened by photoevaporation. We find that below 0.15\,M$_{\odot}$, rapid clearing can happen within $\sim$100\,AU. For higher masses, rapid clearing happens at about 200\,AU irrespective of the stellar mass, up to at least 1\,M$_{\odot}$  \\
---
> \noindent 3) We use the previously established theory of disc photoevaporation to calculate the maximum possible inner hole radius as a function of the stellar mass, for discs with gaps opened by photoevaporation. We find that for discs with an $R^{-1}$ surface density profile, evolving under the effects of photoevaporation alone, thermal sweeping will not initiate until the exponential decrease in density close to the disc outer radius, except at the lowest stellar masses ($\sim0.1$\,M$_{\odot}$). The reason that rapid radiative clearing has been observed in simulations is that the discs considered in such models are constructed manually, without consideration of the photoevaporative history of the disc. Rapid radiative clearing would be important for discs with steeper surface density profiles, such as $R^{-2}$. \\
640c696
< \noindent 4) Since rapid radiative clearing happens less readily than previously believed, the time discs spend in the non--accreting phase will be longer than estimates such as those by \cite{2015arXiv150904278R}. We re-process the population synthesis models from Owen et al. (2011) to calculate the time spent as non--accretors and the maximum inner hole radii of discs. 
---
> \noindent 4) Since rapid radiative clearing happens much less readily than previously believed, the time discs spend in the non--accreting phase will be longer than estimates such as those by \cite{2015arXiv150904278R}. We re-process the population synthesis models from Owen et al. (2011) to calculate the time spent as non--accretors and the maximum inner hole radii of discs. 
656c712
< 	n_{\textrm{D}} = n_{\textrm{\textrm{max}}}\left(\frac{R}{R_{\textrm{\textrm{max}}}}\right)^{-9/4}
---
> 	n_{\textrm{D}} = n_{\textrm{max}}\left(\frac{R}{R_{\textrm{max}}}\right)^{-9/4}
660c716
< 	T_{\textrm{D}} = \max(T_{1\textrm{\textrm{AU}}}\left(\frac{R}{\textrm{\textrm{AU}}}\right)^{-0.5}, 10)
---
> 	T_{\textrm{D}} = \max(T_{1\textrm{AU}}\left(\frac{R}{\textrm{AU}}\right)^{-0.5}, 10)
688c744
< In order to solve for the conditions we have to iterate over possible reasonable values of $n_{\textrm{X}}$ to calculate $\xi$, $T_{\textrm{X}}$ and $\Delta$. Interior to some radius $R_{\textrm{crit}}$, $n_{\textrm{X}}\Delta$ never drops below $10^{22}$, we are in the column limited case and so we set $n_{\textrm{X}}=10^{22}/\Delta$ by construction, allowing us to calculate the conditions as a function of radius (including $\xi$, $\Delta$, $H$ and therefore $\Delta/H$ assuming vertical isothermality). 
---
> In order to solve for the conditions we have to iterate over possible reasonable values of $n_{\textrm{X}}$ to calculate $\xi$, $T_{\textrm{X}}$ and $\Delta$. Interior to some radius $R_{crit}$, $n_{\textrm{X}}\Delta$ never drops below $10^{22}$, we are in the column limited case and so we set $n_{\textrm{X}}=10^{22}/\Delta$ by construction, allowing us to calculate the conditions as a function of radius (including $\xi$, $\Delta$, $H$ and therefore $\Delta/H$ assuming vertical isothermality). 
690c746
<  Once $n\Delta$ drops below $10^{22}$ we have located the transition to being density limited. From here outwards, the ionisation parameter is some minimum value $\xi_{min}$, which Owen et al. (2013) assumed to be $3\times10^{-7}$, but which we calculate explicitly by using the ionisation parameter at the transition radius. We typically find that $\xi_{min}$ is more like $3-6\times10^{-8}$. We can then calculate the number density as
---
>  Once $n\Delta$ drops below $10^{22}$ we have located the transition to being density limited. From here outwards, the ionisation parameter is some minimum value $\xi_{min}$, which Owen et al. (2013) assumed to be $3\times10^{-7}$, but which we calculate explicitly by using the ionisation parameter at the transition radius. We typically find that $\xi_{min}$ is more like $3\times10^{-8}$. We can then calculate the number density as

